Aligning Text-to-Image Models using Human Feedback

Deep generative models have shown impressive results in text-to-image synthesis. However, current text-to-image models often generate images that are inadequately aligned with text prompts. We propose a fine-tuning method for aligning such models using human feedback, comprising three stages. First, we collect human feedback assessing model output alignment from a set of diverse text prompts. We then use the human-labeled image-text dataset to train a reward function that predicts human feedback. Lastly, the text-to-image model is fine-tuned by maximizing reward-weighted likelihood to improve image-text alignment. Our method generates objects with specified colors, counts and backgrounds more accurately than the pre-trained model. We also analyze several design choices and find that careful investigations on such design choices are important in balancing the alignment-fidelity tradeoffs. Our results demonstrate the potential for learning from human feedback to significantly improve text-to-image models.

==> sections/experiments_backup.tex <==




\begin{table}[t!]
\begin{center}
 % \resizebox{\columnwidth}{!}{
 \small
\begin{tabular}{lc}
\toprule
Category & Examples \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Count} \end{tabular}} 
& {\tt One dog}; $\;$ {\tt Two dogs}; $\;$ {\tt Three dogs}; \\ 
& {\tt Four dogs}; $\;$ {\tt Five dogs}; \\  \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Color} \end{tabular}} 
&  {\tt A green colored dog};  \\
&{\tt A red colored dog};  \\  \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Background} \end{tabular}} 
& {\tt A dog in the forest};\\
& {\tt A dog on the moon};    \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Combination} \end{tabular}} 
&  {\tt Two blue dogs in the forest};  \\ 
& {\tt Five white dogs in the city}; \\
\bottomrule
\end{tabular}
\end{center}
\caption{Examples of text categories.}
\label{table:text_example}
\end{table}


\begin{table}[t!]
\begin{center}
 \small
\begin{tabular}{lclll}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Category} \end{tabular}} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Total \# of} \\ {images} \end{tabular}} 
& \multicolumn{3}{c}{Human feedback (\%)} \\ \cmidrule(lr){3-5}
& &  {Good} & {Bad} & {Skip} \\
\midrule
Count & $6480$ & $34.4$ & $61.0$ & $4.6$ \\
Color & $3480$  & $70.4$ & $20.8$ & $8.8$   \\
Background & $2400$  & $66.9$ & $33.1$ & $0.0$   \\
Combination & $15168$  & $35.8$ & $59.9$ & $4.3$   \\  \midrule
Total & $27528$ & $46.5$ &$48.5$ &$5.0$  \\
\bottomrule
\end{tabular}
\end{center}
\caption{Details of image-text datasets and human feedback.}
\label{table:text_dist}
\end{table}



\begin{figure*} [t!] \centering
\subfigure[Seen text prompt: {\tt Two green dogs on the table.}]
{
\includegraphics[width=0.99\textwidth]{figures/quality_1.pdf}
\label{fig:main_fig_0}} 
% \subfigure[Seen text prompt: {\tt Two purple backpacks on the table.}]
% {\includegraphics[width=0.99\textwidth]{figures/quality_2.pdf}
% \label{fig:main_fig_1}}
\subfigure[Unseen text prompt (unseen object): {\tt Five brown bears in the forest.}]
{\includegraphics[width=0.99\textwidth]{figures/quality_3.pdf}
\label{fig:main_fig_2}}
\subfigure[Unseen text prompt (artistic generation): {\tt Oil painting of sunflowers.}]
{\includegraphics[width=0.99\textwidth]{figures/quality_4.pdf}
\label{fig:main_fig_3}}
\caption{Samples from the original Stable Diffusion model (left) and our fine-tuned model (right). (a) Our model generates high-quality seen objects with specified color, count and background. on seen text prompts. 
%(b) Our model generates seen objects with specified color, count and background.
% Even though our human dataset does not contain any image-text samples about {\tt bear},
(b) Our model generates an unseen object ({\tt bear}) with specified color, count, and background. (c) Our model still generates reasonable images from unseen text categories (artistic generation).}
\label{fig:main_fig}
\end{figure*}



\section{Experiments} \label{sec:exp}

We describe a set of experiments designed to test the efficacy of our fine-tuning approach with human feedback.

\subsection{Experimental Setup}

\paragraph{Models.}
%
For our baseline generative model, 
we 
%wstart with
use
stable diffusion v1.5~\cite{stablediffusion}, which has been pre-trained on large image-text datasets~\cite{laion400m,laion-5b}.\footnote{Our fine-tuning method can be used readily with other text-to-image models, such as Imagen~\cite{imagen}, Parti~\cite{parti} and Dalle-2~\cite{dalle2}.} For fine-tuning, we freeze the CLIP language encoder~\cite{clip} and fine-tune only the diffusion module.
For the reward model, we use ViT-L/14 CLIP model~\cite{clip} to extract image and text embeddings and train a MLP using these embeddings as input. More experimental details (e.g., model architectures and the final hyperparameters) are reported in Appendix~\ref{app:exp_detail}.

\paragraph{Datasets.} 
%
From a set of 2700 English prompts (see Table~\ref{table:text_example} for examples), we generate 27K images using the stable diffusion model (see Appendix~\ref{app:dataset} for further details).
% on the prompts and image generation). 
Table~\ref{table:text_dist} shows the feedback distribution provided by multiple human labelers, which has been class-balanced. We note that the stable diffusion model struggles to generate the number of objects specified by the prompt, but reliably generates specified colors and backgrounds.

We use 23K samples for training, with the remaining samples used for validation. 
%\textcolor{red}{We remark that validation set consists of unseen images from seen text prompts and unseen text prompts with seen objects (i.e., interpolation) and unseen objects (i.e., extrapolation)}.
We also use 16K unlabeled samples for the reward-weighted loss
% (the first term in~\eqref{eq:text-to-image-loss}), 
and a 625K subset\footnote{\url{https://huggingface.co/datasets/ChristophSchuhmann/improved_aesthetics_6.5plus}} of LAION-5B~\cite{laion-5b} filtered by an aesthetic score predictor \footnote{\url{https://github.com/christophschuhmann/improved-aesthetic-predictor}} for the pre-training loss.
%for the pre-training loss.
% (the second term in~\eqref{eq:text-to-image-loss}).

% One can note that our dataset is class-balanced.
% \KM{How to split training/validation}






% \begin{figure*} [t!] \centering
% \includegraphics[width=.9\textwidth]{figures/quality.pdf}
% \caption{Samples from the original Stable Diffusion model and our fine-tuned model. (a-c) Our fine-tuned model can generate seen and unseen objects with specified colors, counts and background, i.e., aligned with unseen text prompts. (d) Our model still can generate reasonable images from unseen text prompt under 
% The first row shows. At the same time, fine-tuned model still can generate reasonable image outputs }
% \label{fig:compare_img}
% \end{figure*}







\begin{figure*} [t!] \centering
\subfigure[Seen text prompts]
{\includegraphics[width=0.48\textwidth]{figures/re_human_eval_seen.pdf}
\label{fig:main_seen}} 
\subfigure[Unseen text prompts]
{\includegraphics[width=0.48\textwidth]{figures/re_human_eval_unseen.pdf}
\label{fig:main_unseen}}
\vspace{-0.1in}
\caption{Human evaluation results on (a) 50 seen text prompts and (b) 50 unseen text prompts consisting of unseen objects.
We generate two images (one from our fine-tuned model and one from the original model) with same text prompt. Then, human raters indicate which one is better, or tie (i.e., two images are similar) in terms of image-text alignment and image fidelity. Each query is evaluated by 9 independent human raters and we report the percentage of queries based on the number of positive votes. We also highlight the percentage of queries with two-thirds vote (7 or more positive votes) in the black box.}


%We measure human preference between our fine-tuned model and the original model (i.e., Stable Diffusion) in terms for image-text alignment and image fidelity. 
%The results show the mean and standard deviation averaged over seven independent human raters.}
\label{fig:main}
\end{figure*}

\begin{figure*} [t!] \centering
\subfigure[Comparison with CLIP score~\cite{clip}]
{
\includegraphics[width=0.43\textwidth]{figures/reward.pdf}
\label{fig:comp_clip}} 
\subfigure[Performance of reward function versus data size]
{\includegraphics[width=0.43\textwidth]{figures/reward_frac.pdf}
\label{fig:human_size}}
\vspace{-0.1in}
\caption{(a) Accuracy of CLIP score~\cite{clip} and our reward functions on predicting the preferences of human labelers. For our method, we consider a variant of our reward function, which is not trained with prompt classification (PC) loss in \eqref{eq:pc}. (b) Performance of reward functions with varying the size of the training dataset.}
%\caption{Comparison between fine-tuned Stable Diffusion (ours) and pre-trained Stable Diffusion model on text prompts. We report user preference rates for image-text alignment and image fidelity.}
\label{fig:reward}
\end{figure*}


\begin{figure*} [t!] \centering
\subfigure[Fine-tuned model only with human-labeled dataset.]
{
\includegraphics[width=0.99\textwidth]{figures/compare_1.pdf}
\label{fig:abl_fig_0}} 
\subfigure[Fine-tuned model with human-labeled and unlabeled datasets.]
%\subfigure[Unseen objects with unseen combination: {\tt Three brown bears in the forest.}]
{\includegraphics[width=0.99\textwidth]{figures/compare_2.pdf}
\label{fig:abl_fig_1}}
\subfigure[Fine-tuned model with human-labeled, unlabeled and pre-training datasets.]
{\includegraphics[width=0.99\textwidth]{figures/compare_3.pdf}
\label{fig:abl_fig_2}}
\vspace{-0.1in}
\caption{Samples from fine-tuned models trained with different datasets on unseen text prompts. (a) Fine-tuned model only with human dataset generates low-quality images due to overfitting. (b) Unlabeled samples improve the quality of generated images. (c) Fine-tuned model can generate high-fidelity images by utilizing pre-training dataset.}
\label{fig:abl_fig}
\end{figure*}

% \subsection{Main Results} \label{sec:main_result}
\subsection{Alignment Results} \label{sec:main_result}

% {\bf Human evaluation on tested text prompts}. 
\paragraph{Human evaluation.}
%
We measure human ratings of image alignment with 100 text prompts, testing the ability of the models to render different colors, number of objects, and backgrounds (see Appendix~\ref{app:dataset} for the full set of prompts). 
Given two (anonymized) sets of images, one from our fine-tuned model and one from the stable diffusion model, we ask human raters to assess which is better w.r.t.\ image-text alignment and fidelity (i.e., image quality).\footnote{We ask raters to declare a {\em tie} if they have similar quality.} Each query is evaluated by 9 independent human raters. We show the percentage of queries based on the number of positive votes.
%\textcolor{red}{Each pair is judged by XX independent human raters.}

Figure~\ref{fig:main} shows human evaluation results.
% against the original model. 
Our method significantly improves image-text alignment on both seen (Figure~\ref{fig:main_seen}) and unseen (Figure~\ref{fig:main_unseen}) text prompts.\footnote{Here, ``unseen'' text prompts consist of ``unseen'' objects, which are not in our human dataset.}
Specifically, 59\% and 50\% of samples from our model receive at least two-thirds vote (7 or more positive votes) for image-text alignment.
%w.r.t. our human dataset, i.e., they are not included in the human dataset but pre-training dataset would contain them.} 
%while keeping the similar image quality with the original model on 50 seen text prompts (Figure~\ref{fig:main_seen}). Notably, the gains in alignment still persist even for unseen text prompts consisting of unseen objects (Figure~\ref{fig:main_unseen}).
However, fine-tuning somewhat degrades image fidelity on unseen text prompts (the original model is preferred with two-thirds vote 16 percent of the time). This phenomenon, which is akin to the {\em alignment tax} in language models~\cite{,askell2021general,instructGPT}, is not surprising because (i) we asked the labelers to provide feedback mainly on alignment, (ii) the diversity of our human data is limited, and (iii) we used a small subset of pre-training dataset for fine-tuning. This issue can presumably be mitigated with larger rater and pre-training datasets. 

\paragraph{Qualitative comparison.} 
%
Figure~\ref{fig:main_fig} shows image samples from the original model and our fine-tuned counterpart (see Appendix~\ref{app:example} for more image examples). While the original often generates images with missing details (e.g., color, background or count) (Figure~\ref{fig:main_fig_0}), our model generates objects that adhere to the prompt-specified colors, counts and backgrounds.
Of special note, our model generates high-quality images on unseen text prompts that specify unseen objects (Figure~\ref{fig:main_fig_2}).
Our model also generates reasonable images given unseen text categories, such as artistic generation (Figure~\ref{fig:main_fig_3}).

% \HL{I think we also need human evaluation results.}

% \begin{figure} [t] \centering
% \includegraphics[width=.45\textwidth]{figures/reward.pdf}
% \caption{Performance of CLIP score~\cite{clip} and our reward functions on unseen images from various text prompts.}
% \label{fig:reward}
% \end{figure}





\subsection{Results on Reward Learning}

\paragraph{Predicting human preferences.} 
%
We investigate the quality of our learned reward function by evaluating its prediction of with human ratings. Given two images from the same text prompt $(\img_1,\img_2,\txt)$, we check whether our reward $r_\phi$ generates a higher score for the human-preferred image, i.e., $r_\phi(\img_1, \txt) > r_\phi(\img_2, \txt)$ when rater prefers $\img_1$. As a baseline, we compare it with the CLIP score~\cite{hessel2021clipscore}, which measures image-text similarity in the CLIP embedding space~\cite{clip}.

Figure~\ref{fig:comp_clip} compares the accuracy of $r_\phi$ and the CLIP score on unseen images from both seen and unseen text prompts. Our reward (green) more accurately predicts human evaluation than the CLIP score (red), hence is better aligned with typical human intent.
% and can capture image-text alignment. 
To show the benefit of our auxiliary loss (prompt classification) in \eqref{eq:pc}, we also assess a variant of our reward function which ignores the auxiliary loss (blue). 
The auxiliary  classification task improves reward performance  on both seen and unseen text prompts.
%One can note the performance gain due to our auxiliary task is very significant in improving the generalization ability of reward function.
This clearly shows the importance of text diversity and our auxiliary loss in improving data efficiency.
%benefit of data augmentation and auxiliary task in improving data efficiency.
Although our reward function is more accurate than the CLIP score, its performance on unseen text prompts ($\sim 80\%$) suggests that it may be necessary to use more diverse and large human datasets.
% to be developed.

% Even though our reward function achieves higher accuracy than CLIP score, the performance is roughly 80\% on unseen prompts with unseen objects. 
% We believe that more human data is required to further improve the performance of reward function. 




\begin{figure*} [t!] \centering
\subfigure[Original model versus Rejection sampling]
{
\includegraphics[width=0.48\textwidth]{figures/re_rejection.pdf}
\label{fig:rejection_1}} 
\subfigure[Fine-tuned model versus Rejection sampling]
{\includegraphics[width=0.48\textwidth]{figures/re_rejection_vs_ours.pdf}
\label{fig:rejection_2}}
\caption{Human evaluation on 100 tested text prompts. % (50 seen text prompts and 50 unseen text prompts). 
We generate two images (one from our fine-tuned model and one from the original model) with same text prompt. Then, human raters indicate which one is better, or tie (i.e., two images are similar) in terms for image-text alignment and image fidelity. Each query is evaluated by 9 independent human raters and we report the percentage of queries based on the number of positive votes. We also highlight the percentage of queries with two-thirds vote (7 or more positive votes) in the black box.
(a) For rejection sampling, we generate 16 images per text prompt and select best 4 images based on reward score, i.e., more inference-time compute. (b) Comparison between fine-tuned model and original model with rejection sampling. }
\label{fig:rejection}
\end{figure*}

\paragraph{Rejection sampling.} 
%
Similar to Parti~\cite{parti} and DALL-E~\cite{dalle1}, we evaluate a rejection sampling technique, which selects the best output w.r.t.\ the learned reward function.\footnote{Parti and DALL-E use similarity scores of image and text embeddings from CoCa~\cite{yu2022coca} and CLIP~\cite{clip}, respectively.}
Specifically, we generate 16 images per text prompt from the original stable diffusion model and select the 4 with the highest reward scores. We compare these to 4 randomly sampled images in Figure~\ref{fig:rejection_1}. 
Rejection sampling significantly improves image-text alignment (51\% with two-thirds preference vote by raters) without sacrificing image fidelity. This result illustrates the significant value of the reward function in improving text-to-image models \emph{without any fine-tuning}. 

We also compare our fine-tuned model to the original with rejection sampling in Figure~\ref{fig:rejection_2}.\footnote{We remark that rejection sampling can also be applied on top of our fine-tuned model.} 
Our fine-tuned model achieves a 10\% gain in image-text alignment (22\%-12\% two-thirds vote) without sacrificing image fidelity (6\%-5\% two-thirds vote).
We expect that it would be possible to further improve the performance of fine-tuned models with larger fine-tuning datasets and better hyper-parameters as discussed in Section~\ref{sec:main_result}.
% However, as discussed in Section~\ref{sec:main_result}, we expect degradation in fidelity to be mitigated 
Note also that rejection sampling has several drawbacks, including increased inference-time computation and the inability to improve the model (since it is output post-processing).
%\MGH{What does this written in the parentheses mean?}
% , i.e., hard to improve the model itself.

%However, we think rejection sampling has some limitations in that it corresponds to output post-processing and uses more inference-time compute.


\subsection{Ablation Studies}


\paragraph{Effects of human dataset size.}
%
To investigate how human data quality affects reward learning, we conduct an ablation study,
reducing the number of images per text prompt by half before training the reward function. 
Figure~\ref{fig:human_size} shows that model accuracy decreases on both seen and unseen prompts as data size decreases, clearly demonstrating the importance of diversity and the amount of rater data.

% size of human data
% as the data size decreases, showing the importance of size of human data. We also remark that the performance drop on unseen prompts is bit marginal compared to that on seen prompts. This implies that diversity of text prompts is more important than diversity of images to improve the performance on unseen text prompts. 


\paragraph{Effects of using diverse datasets.}
To verify the importance of data diversity, we incrementally include unlabeled and pre-training datasets during fine-tuning.
% For quantitative evaluation,
We measure the reward score (image-text alignment) on 100 tested text prompts and FID score~\cite{fid}---the similarity between generated images and real images---on MS-CoCo validation data~\cite{mscoco}.
Table~\ref{table:coco_reward} shows that FID score is significantly reduced when the model is fine-tuned using only human data, despite better image-text alignment.
However, by adding the unlabeled and pre-training datasets, FID score is improved without impacting image-text alignment.
We provide image samples from unseen text prompts in Figure~\ref{fig:abl_fig}. We see that fine-tuned models indeed generate more natural images when exploiting more diverse datasets.
% This result clearly shows that diversity of training datasets is very important to improve both image-text alignment and image fidelity. 


% Even though image-text alignment is improved, fine-tuned model only with human datasets generates low-quality images due to lack of diversity of training dataset (Figure~\ref{fig:abl_fig_0}). 
% However, by additionally utilizing unlabeled dataset (Figure~\ref{fig:abl_fig_1}) and pre-training dataset (Figure~\ref{fig:abl_fig_2}), image quality is further improved.
% This result clearly shows that diversity of training datasets is very important to improve both image-text alignment and image fidelity. 





%

% \begin{figure} [t] \centering
% \includegraphics[width=.45\textwidth]{figures/rejection.pdf}
% \caption{Comparison between original model and original model with rejection sampling on 100 tested text prompts (50 seen text prompts and 50 unseen text prompts). For rejection sampling, we generate 16 images per text prompt and select best 4 images based on reward score, i.e., more inference-time compute. The results show the mean and standard deviation averaged over \textcolor{red}{four} independent human raters.}
% \label{fig:rejection}
% \end{figure}




\begin{table}[t]
\begin{center}
 \small
\begin{tabular}{ccc}
\toprule
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} FID on \\ {MS-CoCo} \end{tabular}} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Average rewards on \\ tested text prompts \end{tabular}}  \\
& & \\ \midrule
Original model & $13.97$  & $0.43$   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Fine-tuned model without \\   unlabeled \& pre-train \end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  $26.59$  \end{tabular}}  &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}   $0.62$ \end{tabular}}  \\ 
 &&\\ \midrule
 \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Fine-tuned model \\  without pre-train \end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  $21.02$  \end{tabular}}  &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}   $0.69$ \end{tabular}}  \\
 &&\\  \midrule
Fine-tuned model & $16.76$ &$0.62$   \\
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison with the original Stable Diffusion. For evaluating image fidelity, we measure FID scores on the MS-CoCo. For evaluating the image-text alignment, we measure reward scores and CLIP scores on 100 tested text prompts}
\label{table:coco_reward}
\end{table}


% {\bf Results on MS-CoCo}.
% To investigate the performance of fine-tuned model on the standard benchmark,
% we also measure FID score~\cite{fid}, which calculates the similarity between generated images and real images, on MS-CoCo validation data~\cite{mscoco}.
% %(i.e., val2017) for evaluating the quality of images generated by the original Stable Diffusion model and our fine-tuned model. 
% \textcolor{red}{As shown in Table~\ref{table:coco_reward}, the FID score for the original Stable Diffusion model is 23.78 and that for our fine-tuned model is 27.33.}
% Similar to observations in Figure~\ref{fig:main},
% our fine-tunded model suffers from a performance degradation on image fidelity. 
% We expect that this {\em alignment tax} problem can be mitigated by utilizing larger pre-training dataset during fine-tuning.  
% %Fine-tuning achieves better prompt alignment at the expense of slightly degraded image quality.



==> sections/experiments_submission.tex <==
\begin{table}[t!]
\begin{center}
 % \resizebox{\columnwidth}{!}{
 \small
\begin{tabular}{lc}
\toprule
Category & Examples \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Count} \end{tabular}} 
& {\tt One dog}; $\;$ {\tt Two dogs}; $\;$ {\tt Three dogs}; \\ 
& {\tt Four dogs}; $\;$ {\tt Five dogs}; \\  \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Color} \end{tabular}} 
&  {\tt A green colored dog};  \\
&{\tt A red colored dog};  \\  \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Background} \end{tabular}} 
& {\tt A dog in the forest};\\
& {\tt A dog on the moon};    \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Combination} \end{tabular}} 
&  {\tt Two blue dogs in the forest};  \\ 
& {\tt Five white dogs in the city}; \\
\bottomrule
\end{tabular}
\end{center}
\caption{Examples of the text categories.}
\label{table:text_example}
\end{table}


\begin{table}[t!]
\begin{center}
 \small
\begin{tabular}{lclll}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Category} \end{tabular}} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {Total \# of} \\ {images} \end{tabular}} 
& \multicolumn{3}{c}{Human feedback (\%)} \\ \cmidrule(lr){3-5}
& &  {Good} & {Bad} & {Skip} \\
\midrule
Count & $6480$ & $34.4$ & $61.0$ & $4.6$ \\
Color & $3480$  & $70.4$ & $20.8$ & $8.8$   \\
Background & $2400$  & $66.9$ & $33.1$ & $0.0$   \\
Combination & $15168$  & $35.8$ & $59.9$ & $4.3$   \\  \midrule
Total & $27528$ & $46.5$ &$48.5$ &$5.0$  \\
\bottomrule
\end{tabular}
\end{center}
\caption{Details of image-text datasets and human feedback.}
\label{table:text_dist}
\end{table}



\begin{figure*} [t!] \centering
\subfigure[Seen text prompt: {\tt Two green dogs on the table.}]
{
\includegraphics[width=0.99\textwidth]{figures/quality_1.pdf}
\label{fig:main_fig_0}} 
% \subfigure[Seen text prompt: {\tt Two purple backpacks on the table.}]
% {\includegraphics[width=0.99\textwidth]{figures/quality_2.pdf}
% \label{fig:main_fig_1}}
\subfigure[Unseen text prompt (unseen object): {\tt Five brown bears in the forest.}]
{\includegraphics[width=0.99\textwidth]{figures/quality_3.pdf}
\label{fig:main_fig_2}}
\subfigure[Unseen text prompt (artistic generation): {\tt Oil painting of sunflowers.}]
{\includegraphics[width=0.99\textwidth]{figures/quality_4.pdf}
\label{fig:main_fig_3}}
\caption{Samples from the original Stable Diffusion model (left) and our fine-tuned model (right). (a) Our model generates high-quality seen objects with specified color, count and backgrond. on seen text prompts. 
%(b) Our model generates seen objects with specified color, count and background.
% Even though our human dataset does not contain any image-text samples about {\tt bear},
(b) Our model generates an unseen object ({\tt bear}) with specified color, count, and background. (c) Our model still generates reasonable images from unseen text categories (artistic generation).}
\label{fig:main_fig}
\end{figure*}



\section{Experiments} \label{sec:exp}

We describe a set of experiments designed to test the efficacy of our fine-tuning approach with human feedback.

\subsection{Experimental Setup}

\paragraph{Models.}
%
For our baseline generative model, 
we 
%wstart with
use
stable diffusion v1.5~\cite{stablediffusion}, which has been pre-trained on large image-text datasets~\cite{laion400m,laion-5b}.\footnote{Our fine-tuning method can be used readily with other text-to-image models, such as Imagen~\cite{imagen}, Parti~\cite{parti} and Dalle-2~\cite{dalle2}.} For fine-tuning, we freeze the CLIP language encoder~\cite{clip} and fine-tune only the diffusion module.
For the reward model, we use ViT-L/14 CLIP model~\cite{clip} to extract image and text embeddings and train a MLP using these embeddings as input. More experimental details (e.g., model architectures and the final hyperparameters) are reported in Appendix~\ref{app:exp_detail}.

\paragraph{Datasets.} 
%
From a set of 2700 diverse English prompts (see Table~\ref{table:text_example} for examples), we generate 27K images using the stable diffusion model (see Appendix~\ref{app:dataset} for further details).
% on the prompts and image generation). 
Table~\ref{table:text_dist} shows the feedback distribution provided by multiple human labelers, which has been class-balanced. We note that the stable diffusion model struggles to generate the number of objects specified by the prompt, but reliably generates specified colors and backgrounds.

We use 23K samples for training, with the remaining samples used for validation. 
%\textcolor{red}{We remark that validation set consists of unseen images from seen text prompts and unseen text prompts with seen objects (i.e., interpolation) and unseen objects (i.e., extrapolation)}.
We also use 16K unlabeled samples for the reward-weighted loss
% (the first term in~\eqref{eq:text-to-image-loss}), 
and a 625K subset\footnote{\url{https://huggingface.co/datasets/ChristophSchuhmann/improved_aesthetics_6.5plus}} of LAION-5B~\cite{laion-5b} filtered by an aesthetic score predictor \footnote{\url{https://github.com/christophschuhmann/improved-aesthetic-predictor}} for the pre-training loss.
%for the pre-training loss.
% (the second term in~\eqref{eq:text-to-image-loss}).

% One can note that our dataset is class-balanced.
% \KM{How to split training/validation}






% \begin{figure*} [t!] \centering
% \includegraphics[width=.9\textwidth]{figures/quality.pdf}
% \caption{Samples from the original Stable Diffusion model and our fine-tuned model. (a-c) Our fine-tuned model can generate seen and unseen objects with specified colors, counts and background, i.e., aligned with unseen text prompts. (d) Our model still can generate reasonable images from unseen text prompt under 
% The first row shows. At the same time, fine-tuned model still can generate reasonable image outputs }
% \label{fig:compare_img}
% \end{figure*}







\begin{figure*} [t!] \centering
\subfigure[Seen text prompts]
{\includegraphics[width=0.43\textwidth]{figures/human_eval_seen.pdf}
\label{fig:main_seen}} 
\subfigure[Unseen text prompts]
{\includegraphics[width=0.43\textwidth]{figures/human_eval_unseen.pdf}
\label{fig:main_unseen}}
\caption{Human evaluation results on (a) 50 seen text prompts and (b) 50 unseen text prompts consisting of unseen objects. We measure human preference rates between our fine-tuned model and the original model (i.e., Stable Diffusion) in terms for image-text alignment and image fidelity. The results show the mean and standard deviation averaged over seven independent human raters.}
\label{fig:main}
\end{figure*}

\begin{figure*} [t!] \centering
\subfigure[Comparison with CLIP score~\cite{clip}]
{
\includegraphics[width=0.43\textwidth]{figures/reward.pdf}
\label{fig:comp_clip}} 
\subfigure[Performance of reward function versus data size]
{\includegraphics[width=0.43\textwidth]{figures/reward_frac.pdf}
\label{fig:human_size}}
\caption{(a) Accuracy of CLIP score~\cite{clip} and our reward functions on predicting the preferences of human labelers. For our method, we consider a variant of reward function, which is not trained with preference classification (PC) loss in \eqref{eq:pc}. (b) Performance of reward functions with varying the size of training data.}
%\caption{Comparison between fine-tuned Stable Diffusion (ours) and pre-trained Stable Diffusion model on text prompts. We report user preference rates for image-text alignment and image fidelity.}
\label{fig:reward}
\end{figure*}


\begin{figure*} [t!] \centering
\subfigure[Fine-tuned model only with human-labeled dataset.]
{
\includegraphics[width=0.99\textwidth]{figures/compare_1.pdf}
\label{fig:abl_fig_0}} 
\subfigure[Fine-tuned model with human-labeled and unlabeled datasets.]
%\subfigure[Unseen objects with unseen combination: {\tt Three brown bears in the forest.}]
{\includegraphics[width=0.99\textwidth]{figures/compare_2.pdf}
\label{fig:abl_fig_1}}
\subfigure[Fine-tuned model with human-labeled, unlabeled and pre-training datasets.]
{\includegraphics[width=0.99\textwidth]{figures/compare_3.pdf}
\label{fig:abl_fig_2}}
\caption{Samples from fine-tuned models trained with different datasets on unseen text prompts. (a) Fine-tuned model only with human dataset generates low-quality images due to overfitting. (b) Unlabeled samples improve the quality of generated images. (c) Fine-tuned model can generate high-fidelity images by utilizing pre-training dataset.}
\label{fig:abl_fig}
\end{figure*}

% \subsection{Main Results} \label{sec:main_result}
\subsection{Alignment Results} \label{sec:main_result}

% {\bf Human evaluation on tested text prompts}. 
\paragraph{Human evaluation.}
%
We measure human ratings of image alignment with 100 text prompts, testing the ability of the models to render different colors, number of objects, and backgrounds (see Appendix~\ref{app:dataset} for the full set of prompts). 
Given two (anonymized) sets of images, one from our fine-tuned model and one from the stable diffusion model, we ask human raters to assess which is better w.r.t.\ image-text alignment and fidelity (i.e., image quality).\footnote{We ask raters to declare a {\em tie} if they have similar quality.}
%\textcolor{red}{Each pair is judged by XX independent human raters.}

Figure~\ref{fig:main} shows Win-Lose-Tie rates of both models.
% against the original model. 
Our method significantly improves image-text alignment on both seen (Figure~\ref{fig:main_seen}) and unseen (Figure~\ref{fig:main_unseen}) text prompts.\footnote{Here, ``unseen'' text prompts consist of ``unseen'' objects, which are not in our human dataset.}
%w.r.t. our human dataset, i.e., they are not included in the human dataset but pre-training dataset would contain them.} 
%while keeping the similar image quality with the original model on 50 seen text prompts (Figure~\ref{fig:main_seen}). Notably, the gains in alignment still persist even for unseen text prompts consisting of unseen objects (Figure~\ref{fig:main_unseen}).
However, fine-tuning somewhat degrades image fidelity. This phenomenon, which is akin to the {\em alignment tax} in language models~\cite{,askell2021general,instructGPT}, is not surprising because (i) we asked the labelers to provide feedback mainly on alignment, (ii) the diversity of our human data is limited, and (iii) we used a small subset of pre-training dataset for fine-tuning. This issue can presumably be mitigated with larger rater and pre-training datasets. 

\paragraph{Qualitative comparison.} 
%
Figure~\ref{fig:main_fig} shows image samples from the original model and our fine-tuned counterpart (see Appendix~\ref{app:example} for more image examples). While the original often generates images with missing details (e.g., color, background or count) (Figure~\ref{fig:main_fig_0}), our model generates objects that adhere to the prompt-specified colors, counts and backgrounds.
Of special note, our model generates high-quality images on unseen text prompts that specify unseen objects (Figure~\ref{fig:main_fig_2}).
Our model also generates reasonable images given unseen text categories, such as artistic generation (Figure~\ref{fig:main_fig_3}).

% \HL{I think we also need human evaluation results.}

% \begin{figure} [t] \centering
% \includegraphics[width=.45\textwidth]{figures/reward.pdf}
% \caption{Performance of CLIP score~\cite{clip} and our reward functions on unseen images from various text prompts.}
% \label{fig:reward}
% \end{figure}





\subsection{Results on Reward Learning}

\paragraph{Predicting human preferences.} 
%
We investigate the quality of our learned reward function by evaluating its prediction of with human ratings. Given two images from the same text prompt $(\img_1,\img_2,\txt)$, we check whether our reward $r_\phi$ generates a higher score for the human-preferred image, i.e., $r_\phi(\img_1, \txt) > r_\phi(\img_2, \txt)$ when rater prefers $\img_1$. As a baseline, we compare it with the CLIP score~\cite{hessel2021clipscore}, which measures image-text similarity in the CLIP embedding space~\cite{clip}.

Figure~\ref{fig:comp_clip} compares the accuracy of $r_\phi$ and the CLIP score on unseen images from both seen and unseen text prompts. Our reward (green) more accurately predicts human evaluation than the CLIP score (red), hence is better aligned with typical human intent.
% and can capture image-text alignment. 
To show the benefit of our auxiliary loss (prompt classification) in \eqref{eq:pc}, we also assess a variant of our reward function which ignores the auxiliary loss (blue). 
The auxiliary  classification task improves reward performance  on both seen and unseen text prompts.
%One can note the performance gain due to our auxiliary task is very significant in improving the generalization ability of reward function.
This clearly shows the importance of text diversity and our auxiliary loss in improving data efficiency.
%benefit of data augmentation and auxiliary task in improving data efficiency.
Although our reward function is more accurate than the CLIP score, its performance on unseen text prompts ($\sim 80\%$) suggests the use of more diverse and larger human datasets.
% to be developed.

% Even though our reward function achieves higher accuracy than CLIP score, the performance is roughly 80\% on unseen prompts with unseen objects. 
% We believe that more human data is required to further improve the performance of reward function. 


\paragraph{Rejection sampling.} 
%
Similar to Parti~\cite{parti} and DALL-E~\cite{dalle1}, we evaluate a rejection sampling technique, which selects the best output w.r.t.\ the learned reward function.\footnote{Parti and DALL-E use similarity scores of image and text embeddings from CoCa~\cite{yu2022coca} and CLIP~\cite{clip}, respectively.}
Specifically, we generate 16 images per text prompt from the original stable diffusion model and select the 4 with the highest reward scores. We compare these to 4 randomly sampled images in Figure~\ref{fig:rejection_1}. 
Rejection sampling significantly improves image-text alignment without sacrificing image fidelity. This result illustrates the significant value of the reward function in improving text-to-image models \emph{without any fine-tuning}. 

We also compare our fine-tuned model to the original with rejection sampling in Figure~\ref{fig:rejection_2}. Our fine-tuned model achieves a 13\% gain in image-text alignment (25\%-12\% win-loss rate) but sacrifices 15\% in image fidelity (8\%-23\% win-loss rate).
However, as discussed in Section~\ref{sec:main_result}, we expect degradation in fidelity to be mitigated with larger fine-tuning datasets and better hyper-parameters. Note also that rejection sampling has several drawbacks, including increased inference-time computation and the inability to improve the model (since it is output post-processing).
%\MGH{What does this written in the parentheses mean?}
% , i.e., hard to improve the model itself.

%However, we think rejection sampling has some limitations in that it corresponds to output post-processing and uses more inference-time compute.


\begin{figure*} [t!] \centering
\subfigure[Original model versus Rejection sampling]
{
\includegraphics[width=0.43\textwidth]{figures/rejection.pdf}
\label{fig:rejection_1}} 
\subfigure[Fine-tuned model versus Rejection sampling]
{\includegraphics[width=0.43\textwidth]{figures/rejection_vs_ours.pdf}
\label{fig:rejection_2}}
\caption{Human evaluation on 100 tested text prompts. % (50 seen text prompts and 50 unseen text prompts). 
The results show the mean and standard deviation averaged over four independent human raters. (a) For rejection sampling, we generate 16 images per text prompt and select best 4 images based on reward score, i.e., more inference-time compute. (b) Comparison between fine-tuned model and original model with rejection sampling. }
\label{fig:rejection}
\end{figure*}

\subsection{Ablation Studies}


\paragraph{Effects of human dataset size.}
%
To investigate how human data quality affects reward learning, we conduct an ablation study,
reducing the number of images per text prompt by half before training the reward function. 
Figure~\ref{fig:human_size} shows that model accuracy decreases on both seen and unseen prompts as data size decreases, clearly demonstrating the importance of diversity and the amount of rater data.

% size of human data
% as the data size decreases, showing the importance of size of human data. We also remark that the performance drop on unseen prompts is bit marginal compared to that on seen prompts. This implies that diversity of text prompts is more important than diversity of images to improve the performance on unseen text prompts. 


\paragraph{Effects of using diverse datasets.}
To verify the importance of data diversity, we incrementally include unlabeled and pre-training datasets during fine-tuning.
% For quantitative evaluation,
We measure the reward score (image-text alignment) on 100 tested text prompts and FID score~\cite{fid}---the similarity between generated images and real images---on MS-CoCo validation data~\cite{mscoco}.
Table~\ref{table:coco_reward} shows that FID score is significantly reduced when the model is fine-tuned using only human data, despite better image-text alignment.
However, by adding the unlabeled and pre-training datasets, FID score is improved without impacting image-text alignment.
We provide image samples from unseen text prompts in Figure~\ref{fig:abl_fig}. We see that fine-tuned models indeed generate more natural images when exploiting more diverse datasets.
% This result clearly shows that diversity of training datasets is very important to improve both image-text alignment and image fidelity. 


% Even though image-text alignment is improved, fine-tuned model only with human datasets generates low-quality images due to lack of diversity of training dataset (Figure~\ref{fig:abl_fig_0}). 
% However, by additionally utilizing unlabeled dataset (Figure~\ref{fig:abl_fig_1}) and pre-training dataset (Figure~\ref{fig:abl_fig_2}), image quality is further improved.
% This result clearly shows that diversity of training datasets is very important to improve both image-text alignment and image fidelity. 





%

% \begin{figure} [t] \centering
% \includegraphics[width=.45\textwidth]{figures/rejection.pdf}
% \caption{Comparison between original model and original model with rejection sampling on 100 tested text prompts (50 seen text prompts and 50 unseen text prompts). For rejection sampling, we generate 16 images per text prompt and select best 4 images based on reward score, i.e., more inference-time compute. The results show the mean and standard deviation averaged over \textcolor{red}{four} independent human raters.}
% \label{fig:rejection}
% \end{figure}




\begin{table}[t]
\begin{center}
 \small
\begin{tabular}{ccc}
\toprule
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} FID on \\ {MS-CoCo} \end{tabular}} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Average rewards on \\ tested text prompts \end{tabular}}  \\
& & \\ \midrule
Original model & $13.97$  & $0.43$   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Fine-tuned model without \\   unlabeled \& pre-train \end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  $26.59$  \end{tabular}}  &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}   $0.62$ \end{tabular}}  \\ 
 &&\\ \midrule
 \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Fine-tuned model \\  without pre-train \end{tabular}} 
 &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  $21.02$  \end{tabular}}  &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}   $0.69$ \end{tabular}}  \\
 &&\\  \midrule
Fine-tuned model & $16.76$ &$0.62$   \\
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison with the original Stable Diffusion. For evaluating image fidelity, we measure FID scores on the MS-CoCo. For evaluating the image-text alignment, we measure reward scores and CLIP scores on 100 tested text prompts}
\label{table:coco_reward}
\end{table}


% {\bf Results on MS-CoCo}.
% To investigate the performance of fine-tuned model on the standard benchmark,
% we also measure FID score~\cite{fid}, which calculates the similarity between generated images and real images, on MS-CoCo validation data~\cite{mscoco}.
% %(i.e., val2017) for evaluating the quality of images generated by the original Stable Diffusion model and our fine-tuned model. 
% \textcolor{red}{As shown in Table~\ref{table:coco_reward}, the FID score for the original Stable Diffusion model is 23.78 and that for our fine-tuned model is 27.33.}
% Similar to observations in Figure~\ref{fig:main},
% our fine-tunded model suffers from a performance degradation on image fidelity. 
% We expect that this {\em alignment tax} problem can be mitigated by utilizing larger pre-training dataset during fine-tuning.  
% %Fine-tuning achieves better prompt alignment at the expense of slightly degraded image quality.


